Open Set Recognition with Conditional Probabilistic Generative Models

Deep neural networks have made breakthroughs in a wide range of visual understanding tasks. A typical challenge that hinders their real-world applications is that unknown samples may be fed into the system during the testing phase, but traditional deep neural networks will wrongly recognize these unknown samples as one of the known classes. Open set recognition (OSR) is a potential solution to overcome this problem, where the open set classifier should have the flexibility to reject unknown samples and meanwhile maintain high classification accuracy in known classes. Probabilistic generative models, such as Variational Autoencoders (VAE) and Adversarial Autoencoders (AAE), are popular methods to detect unknowns, but they cannot provide discriminative representations for known classification. In this paper, we propose a novel framework, called Conditional Probabilistic Generative Models (CPGM), for open set recognition. The core insight of our work is to add discriminative information into the probabilistic generative models, such that the proposed models can not only detect unknown samples but also classify known classes by forcing different latent features to approximate conditional Gaussian distributions. We discuss many model variants and provide comprehensive experiments to study their characteristics. Experiment results on multiple benchmark datasets reveal that the proposed method significantly outperforms the baselines and achieves new state-of-the-art performance.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sub_content/5_analysis_experiment.tex <==

\begin{table}[t]
\centering

\caption{Comparison of different metric-based methods  for 1-shot classification. Our model with EMD as the distance metric significantly outperforms baseline models based on image-level representations and local representations. }


\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule[1.2pt]
\multicolumn{1}{l}{Model}   & Embedding & Metric  &  5-way &10-way\\ \hline\hline
ProtoNet~\cite{proto} & global &Euclidean &60.37  &44.34         \\ 
MatchingNet~\cite{matchnet}& global  & \emph{cosine} &63.08 &47.09               \\
FC~\cite{closer} & global &  \emph{dot} &59.41      &44.08    \\ 
FC~\cite{closer}  & global & \emph{cosine} &55.43  &40.42         \\ 
\Xhline{1pt}
KNN~\cite{Revisiting}  &local&\emph{cosine}         &62.52&47.08  \\ 
Prediction Fusion~\cite{dense} & local & \emph{cosine} &62.38   &47.04             \\
\textbf{DeepEMD-FCN (our)} &local & EMD & \textbf{65.91} & \textbf{49.66} \\  \Xhline{1.2pt}
\end{tabular}%
}

\label{table:1shotcomparison}
\end{table}




\begin{table}[t]
\centering

\caption{Different methods for setting the weights in the EMD. We report the 1-shot performance with only the feature pre-training step. EMD with our cross-reference (\textbf{CR}) mechanism yields the best result. The model variant that is solely based the on the cross-reference mechanism as attention and removes the EMD can cause a significant performance drop. The combination of the EMD and the cross-reference generates the best result.   }


\small 
\begin{tabular}{lccc}
\toprule[1pt]
\multicolumn{1}{c}{Method}  & Operation & 5-way& 10-way \\ \hline\hline
Full Connections&Average & 55.16  & 40.88         \\ 
Full Connections&\textbf{CR} & 55.41  & 41.60         \\ 
\Xhline{1pt}
EMD&Equal & 56.95  & 42.89         \\ 
EMD&K-means~\cite{kmeans} & 56.25   & 41.85             \\
EMD&mean-shift~\cite{meanshift} & 53.56 & 39.70               \\
EMD& \textbf{CR} & \textbf{61.13}  & \textbf{46.92}              \\
 \Xhline{1.2pt}
\end{tabular}%

\label{table:weights}
\end{table}












\begin{table}[t]
\centering

\caption{Comparison of different local embedding extractors described in Section~\ref{sec:emd}. $\mathbf{P_{feat}}$ denotes the feature pyramid structure applied on DeepEMD-FCN and $\mathbf{P_{grid}}$ denotes the image pyramid structure applied on DeepEMD-Grid. The parameters in $\mathbf{P_{feat}}$ and $\mathbf{P_{grid}}$ are the RoI pooling size and the grid size, respectively. DeepEMD-Sampling outperforms the plain version of other two methods and both pyramid structures in feature level and image level can effectively boost the performance.}


{%
\begin{tabular}{lccc}
\toprule[1pt]
\multicolumn{1}{c}{Method} & Embedding & 5-way& 10-way \\ \hline\hline
\multirow{4}{*}{DeepEMD-FCN}&$5 \times 5$& 65.91  & 49.66         \\ \cline{2-4} 
&$\mathbf{P_{feat}}(5, 3)$  & 66.27  & 49.85         \\ 
&$\mathbf{P_{feat}}(5, 2)$  & 66.42  & 50.02         \\ 
&$\mathbf{P_{feat}}(5, 2, 1)$  & \textbf{66.50}  & \textbf{50.09}         \\ 
\Xhline{0.8pt}
\multirow{9}{*}{DeepEMD-Grid}&$6 \times 6$& 63.61  & 48.72         \\ 
&$5 \times 5$    & 65.38  & 50.08 \\ 
&$4 \times 4$   & 66.57  &  51.42  \\ 
&$3 \times 3$   & 67.31 &	52.26        \\ 
&$2 \times 2$   &66.09 &	50.94 \\ \cline{2-4} 
&$\mathbf{P_{grid}}(3,2 )$    & 67.74 &	52.76 \\ 
&$\mathbf{P_{grid}}(5,3 )$   & 67.01 & 51.89\\ 
&$\mathbf{P_{grid}}(5,2 )$   &  67.39 & 52.20 \\ 
&$\mathbf{P_{grid}}(5,3,2 )$  & \textbf{67.83} & \textbf{52.85} \\ 
\Xhline{0.9pt}
\multirow{3}{*}{DeepEMD-Sampling}&9 patches & 68.09 & 53.04\\ 
& 16 patches & 68.54 & 53.61  
         \\ 
& 25 patches & \textbf{68.77} & \textbf{53.83} 
         \\ 
 \Xhline{1.2pt}
\end{tabular}%
}

\label{table:extractor}
\end{table}


















\begin{table}[t]

\centering


\caption{Cross-domain experiments (\emph{mini}Imagenet $\rightarrow$ CUB). We report the performance with 95\% confidence intervals on 1-shot 5-way and 5-shot 5-way tasks. We use FCN to extract local features for KNN and our method. Our proposed algorithm outperforms baseline methods \textbf{with a large margin.} }

{%
\begin{tabular}{lcc}
\toprule[1.2pt]
\multicolumn{1}{l}{Model}      &  1-shot &5-shot\\ \hline\hline
ProtoNet~\cite{proto}   &50.01 \small{$\pm$ $0.82$}  &72.02 \small{$\pm$ $0.67$}         \\ 
MatchingNet~\cite{matchnet} &51.65 \small{$\pm$ $0.84$}  &69.14 \small{$\pm$ $0.72$}         \\ 
\emph{cosine} classifier~\cite{closer}  &44.17 \small{$\pm$ $0.78$}  &69.01 \small{$\pm$ $0.74$}         \\ 
\emph{linear} classifier~\cite{closer}  &50.37 \small{$\pm$ $0.79$}  &73.30 \small{$\pm$ $0.69$}         \\ 


KNN~\cite{Revisiting}       &50.84 \small{$\pm$ $0.81$}  &71.25 \small{$\pm$ $0.69$}         \\  \Xhline{1pt}
\textbf{DeepEMD-FCN}  &\textbf{54.24} \small{$\pm$ \textbf{0.86}}  &\textbf{78.86} \small{$\pm$ \textbf{0.65}}         \\
\Xhline{1.2pt}
\end{tabular}%
}

\label{table:cross}
\end{table}





\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{pyramid.pdf}
	\caption{Pyramid structures applied on DeepEMD-FCN and DeepEMD-Grid to extract local embeddings. The feature pyramid structure (a) adopts RoI poolings with different output sizes on the feature maps to generate local embeddings at multiple scales while the image pyramid structure (b) crops the input image into patches according to different grid sizes and all patches are sent to the CNN to generate local embeddings.}
	\label{fig:pyramid}
\end{figure}







\begin{table}[t]
\centering

\caption{Computation time of the EMD layer in DeepEMD-FCN. In a 5-way 1-shot task with 10 query images, we vary the spatial size and the feature dimension of two input feature maps and record their computation time. }


\begin{tabular}{cccc}
\toprule[1.2pt]
Solver &Spatial Size   &  Dimension & Time\\ \hline\hline

\multirow{12}{*}{QPTH~\cite{amos2017optnet}} & $3 \times 3$& 256 & 0.294 s        \\ 
& $3 \times 3$ &512 &0.294 s        \\ 
 &$3 \times 3$  &1024  &0.295 s         \\ 
  &$3 \times 3$  &2048  &0.295 s         \\ \cline{2-4} 
 &$4 \times 4$& 256 &1.489 s        \\ 
 &$4 \times 4$ &512 &1.493 s         \\ 
&$4 \times 4$  &1024  &1.498 s         \\ 
& $4 \times 4$  &2048  &1.499 s         \\ \cline{2-4} 
& $5 \times 5$& 256 &8.595 s        \\ 
&$5 \times 5$ &512 &8.638 s          \\ 
& $5 \times 5$  &1024  &8.638 s         \\ 
& $5 \times 5$  &2048  &8.650 s  \\\hline
\multirow{4}{*}{OpenCV~\cite{OpenCV}} & $5 \times 5$& 256 &0.018 s        \\ 
 & $5 \times 5$ &512 &0.019 s          \\ 
& $5 \times 5$  &1024  &0.021 s         \\ 
 & $5 \times 5$  &2048  &0.025 s 
      \\\Xhline{1.2pt}
\end{tabular}%

\label{table:time}
\end{table}


==> zc_5_experiment.tex <==
\section{Experiments}
To evaluate the performance of our proposed algorithm for few-shot classification, we conduct extensive experiments on multiple datasets. In this section, we first present dataset information and some important implementation details in our network design. Then, we conduct various ablative experiments to validate each component in our network. Finally, we compare our model with the state-of-the-art methods on popular benchmark datasets.

\subsection{Implementation Details}
\textbf{Network.} For a fair comparison with previous works, we employ a 10-layer ResNet (ResNet10) as our model backbone, which is widely used in the few-shot classification literature. For DeepEMD-Grid and DeepEMD-Sampling, we remove the fully connected layer in ResNet, such that the network generates a vector for each input image patch. For DeepEMD-FCN, we further remove the global average pooling layer, such that the network is transformed into a  fully convolutional network. Specifically, given an image of size $84\times84$, the model generates a feature map of size $5\times5\times512$, \ie 25 512-dimensional vectors. For DeepEMD-Grid, we slightly enlarge the region of the local patches in the grid by a factor of 2 to incorporate context information, which is found helpful to generate local representations. 

\textbf{Training.} At training time, we 
use 
the GPU accelerated convex optimization solver QPTH~\cite{amos2017optnet} to solve the Linear Programming problem in our network and compute gradients for back-propagation. 
As is commonly implemented in the state-of-the-art literature, we adopt a feature pre-training step followed by the episodic meta-training~\cite{matchnet} to learn our network. In the pre-training stage, we train a standard classification model with all training classes and we use DeepEMD-FCN for validation with the validation set in the training process. After pre-training, the model with the highest validation accuracy is further optimized by episodic training.  
For the \emph{k}-shot classification task, we initialize the parameters in structured FC layer with the average local representations of all support data in each class, and sample a mini-batch of 5 images from the support set to finetune the structured FC layer for 100 iterations. 

\subsection{Dataset Description}
We conduct few-shot classification experiments on four popular benchmark datasets: \emph{mini}ImageNet~\cite{matchnet}, \emph{tiered}ImageNet~\cite{tieredimagenet}, Fewshot-CIFAR100 (FC100)~\cite{TADAM} and Caltech-UCSD Birds-200-2011 (CUB)~\cite{cub}.

\textbf{\emph{mini}ImageNet.} \emph{mini}ImageNet was first proposed in~\cite{matchnet}, and becomes the most popular benchmark in the few-shot classification literature. It contains 100 classes with 600 images in each class, which are built upon the ImageNet dataset~\cite{imagenet}. The 100 classes are divided into 64, 16, 20 for meta-training, meta-validation and meta-testing, respectively.

\textbf{\emph{tiered}ImageNet.} \emph{tiered}ImageNet is also a subset of ImageNet, which includes 608 classes from 34 super-classes. Compared with  \emph{mini}ImageNet, the splits of meta-training(20), meta-validation(6) and meta-testing(8) are set according to the super-classes to enlarge the domain difference between  training and testing phase. The dataset also include more images for training and evaluation (779,165 images in total).

 
\textbf{Fewshot-CIFAR100.} FC100 is a few-shot classification dataset build on CIFAR100~\cite{CIFAR100}. We follow the split division proposed in~\cite{TADAM}, where 36 super-classes were divided into 12 (including 60 classes), 4 (including 20 classes), 4 (including 20 classes), for meta-training, meta-validation and meta-testing, respectively, and each class contains 100 images.

\textbf{Caltech-UCSD Birds-200-2011.} CUB was originally proposed for fine-grained bird classification, which contains 11,788 images from 200 classes. We follow the splits in~\cite{feat} that 200 classes are divided into 100, 50 and 50 for meta-training, meta-validation and meta-testing, respectively. The challenge in this dataset is the minor difference between classes.  
\input{sub_content/5_analysis_experiment}


\input{6_1_soatable.tex}

\subsection{Ablation Study of CGDL on VAE}
\label{sec:ablation}
In this section, we analyze our contributions from each component of the proposed method on CIFAR-100 dataset~\cite{cifar100}. The CIFAR-100 dataset consists of 100 classes, containing 500 training images and 100 testing images in each class. For ablation analysis, the performance is measured by F-measure (or F1-scores) \cite{f1} against varying Openness \cite{toward}. Openness is defined as follows:

\begin{equation}
    Openness=1-\sqrt{\frac {2\times N_{train}}{N_{test}+N_{target}}}
\end{equation}
where $N_{train}$ is the number of known classes seen during training, $N_{test}$ is the number of classes that will be observed during testing, and $N_{target}$ is the number of classes to be recognized during testing. We randomly sample 15 classes out of 100 classes as known classes and varying the number of unknown classes from 15 to 85, which means Openness is varied from 18\% to 49\%. The performance is evaluated by the macro-average F1-scores in 16 classes (15 known classes and \emph{unknown}).

\begin{table}
\begin{center}
\begin{tabular}{l c c c c}
\hline
Architecture  & MNIST & SVHN & CIFAR-10\\
\hline\hline
Plain CNN & 0.997 & 0.944 & 0.912\\
\hline
CGDL & 0.996 & 0.942 & 0.912\\
\hline
\end{tabular}
\end{center}
\caption{Comparison of closed set test accuracies between the plain CNN and the proposed method CGDL. Although the training objective of CGDL is classifying known samples as well as learning conditional Gaussian distributions, there is no significant degradation in closed set accuracy.}
\label{close}
\end{table}

We compare the following baselines for ablation analysis:\\
\textbf{I. CNN}: In this baseline, only the encoder ${\mathcal{F}}$ (without ladder architecture) and the known classifier ${\mathcal{C}}$ are trained for closed set classification. This model can be viewed as a traditional convolutional neural network (CNN). During testing, learned features will be fed to ${\mathcal{C}}$ to get the probability scores of known classes. A sample will be recognized as unknown if its probability score of predicted label is less than 0.5.\\
\textbf{II. CVAE}: The encoder ${\mathcal{F}}$, decoder ${\mathcal{G}}$ and classifier ${\mathcal{C}}$ are trained without the ladder architecture, and the testing procedure is the same as baseline I. This model can be viewed as a class conditional variational auto-encoder (CVAE).\\
\textbf{III. LCVAE}: The probabilistic ladder architecture is adopted in the CVAE, which contributes to the KL-divergences during training (Eqn.~\ref{kl}). We call this model as LCVAE. The testing procedure is the same as baseline I and II.\\
\textbf{IV. CVAE+CGD}: The model architecture and training procedure are the same as baseline II, while the conditional Gaussian distributions (CGD) are used to detect unknowns during testing.\\
\textbf{V. LCVAE+CGD}: In this baseline, LCVAE is introduced along with CGD-based unknown detector. The training and testing procedure are respectively the same as baseline III and IV.\\
\textbf{VI. LCVAE+RE}: Different from baseline V, reconstruction errors (RE), instead of CGD, are used in LCVAE to detect unknown samples.\\
\textbf{VII. Proposed Method}: The training procedure is the same as baseline V and VI, while during testing conditional Gaussian distributions and reconstruction errors are together used for unknown detection.\\

The experimental results are shown in Fig.~\ref{fig:abla}. Among baseline I, II and III, unknown detection simply relies on the known classifier ${\mathcal{C}}$. Although the performance is a little improved when the probabilistic ladder architecture is adopted (baseline III), the overall performance in these three baselines is weak as the F1-scores degrade rapidly as the Openness increases. Conditional Gaussian distributions (CGD) is added for unknown detection in CVAE model (baseline IV), but it has seen no visible change in performance. In baseline V, this trend is alleviated by introducing CGD-based unknown detector into LCVAE. This shows the importance of the probabilistic ladder architecture for open set recognition. It is also the reason why the CGD-based unknown detection achieves better performance in baseline V than in baseline IV. If we only use reconstruction errors to detect unknowns (baseline VI), the results are worst. However, if reconstruction errors are added to the CGD-based unknown detector (baseline VII), there is a little improvement in performance. As a result, applying conditional Gaussian distributions and reconstruction errors to detect unknowns with the probabilistic ladder architecture achieves the best performance.






==> zc_6_1_soatable.tex <==































					
				
		
					











						

						












	
	







\begin{table*}[t]

	\caption{ Comparison with the state-of-art 1-shot 5-way and 5-shot 5-way performance (\textbf{\%}) with 95\% confidence intervals on \textbf{\emph{mini}ImageNet }\textbf{(a)}, \textbf{\emph{tiered}ImageNet} \textbf{(a)}, \textbf{Fewshot-CIFAR100  }\textbf{(b)} and \textbf{Caltech-UCSD Birds-200-2011 }\textbf{(c)} datasets. Our model achieves new state-of-the-art performance on all datasets, and even outperforms methods with deeper backbones${}^{\dag}$. }
	
	
	

		\begin{minipage}[t]{1\textwidth}
			\centering
			\begin{subtable}{1\textwidth}
				\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} ccccc @{}}%
					\toprule[1pt]
					\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Backbone}}} & \multicolumn{2}{c}{\textbf{\emph{mini}Imagenet}}                              & \multicolumn{2}{c}{\textbf{\emph{tiered}Imagenet}}                              \\ \Xcline{3-6}{1pt}%

					\multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                          & \multicolumn{1}{c}{\textbf{1-shot}} & \multicolumn{1}{c}{\textbf{5-shot}} & \multicolumn{1}{c}{\textbf{1-shot}} & \multicolumn{1}{c}{\textbf{5-shot}} \\%\midrule[0.5pt]
\Xhline{1pt}


\textbf{\emph{cosine} classifier~\cite{closer}} & \emph{ResNet12}  & 55.43 \small{$\pm$ $0.81$} & 77.18 \small{$\pm$ $0.61$}  & 61.49 \small{$\pm$ $0.91$}  & 82.37. \small{$\pm$ $0.67$} \\


\textbf{TADAM~\cite{TADAM}}  & \emph{ResNet12}  & 58.50 \small{$\pm$ $0.30$} & 76.70 \small{$\pm$ $0.30$}  &  -  &  - \\

\textbf{ECM~\cite{ECM}}  & \emph{ResNet12}  & 59.00 \small{$\pm$ $-$} & 77.46 \small{$\pm$ $-$}  &  63.99 \small{$\pm$ $-$}  &  81.97 \small{$\pm$ $-$} \\

\textbf{TPN~\cite{tpn}}  & \emph{ResNet12}  & 59.46
 \small{$\pm$ $ -$} & 75.65
 \small{$\pm$ $ -$}  & 59.91 \small{$\pm$ $0.94$}  & 73.30 \small{$\pm$ $0.75$} \\

\textbf{PPA~\cite{PPA}}  & \emph{WRN\small{-28-10}}${}^{\dag}$  & 59.60 \small{$\pm$ $0.41$} & 73.74  \small{$\pm$ $0.19$}  & 65.65 \small{$\pm$ $0.92$}  & 83.40. \small{$\pm$ $0.65$} \\


\textbf{ProtoNet~\cite{proto}}  & \emph{ResNet12}  & 60.37 \small{$\pm$ $0.83$} & 78.02 \small{$\pm$ $0.57$}  & 65.65 \small{$\pm$ $0.92$}  & 83.40. \small{$\pm$ $0.65$} \\

\textbf{wDAE-GNN~\cite{wDAE}}  & \emph{WRN\small{-28-10}}${}^{\dag}$  & 61.07 \small{$\pm$ $0.15$} & 76.75 \small{$\pm$ $0.11$}  & 68.18 \small{$\pm$ $0.16$}  & 83.09 \small{$\pm$ $0.12$} \\


\textbf{MTL~\cite{yaoyao}}  & \emph{ResNet12}  & 61.20 \small{$\pm$ $1.80$} & 75.50 \small{$\pm$ $0.80$}  & -  & - \\

\textbf{LEO~\cite{leo}}  & \emph{WRN\small{-28-10}}${}^{\dag}$  & 61.76 \small{$\pm$ $0.08$} & 77.59 \small{$\pm$ $0.12$}  & 66.33 \small{$\pm$ $0.05$}  & 81.44 \small{$\pm$ $0.09$} \\


\textbf{DC~\cite{dense}}  & \emph{ResNet12}  & 62.53 \small{$\pm$ $0.19$} & 79.77 \small{$\pm$ $0.19$}  & - & -\\


\textbf{MetaOptNet~\cite{metaoptnet}}  & \emph{ResNet12}  & 62.64 \small{$\pm$ $0.82$} & 78.63 \small{$\pm$ $0.46$}  & 65.99 \small{$\pm$ $0.72$}  & 81.56 \small{$\pm$ $0.53$} \\

\textbf{FEAT~\cite{feat}}  & \emph{ResNet24}${}^{\dag}$  & 62.96 \small{$\pm$ $0.20$} & 78.49 \small{$\pm$ $0.15$}  & - & - \\


\textbf{MatchNet~\cite{matchnet}}  & \emph{ResNet12}  & 63.08 \small{$\pm$ $0.80$} & 75.99 \small{$\pm$ $0.60$}  & 68.50 \small{$\pm$ $0.92$}  & 80.60 \small{$\pm$ $0.71$} \\

\textbf{CTM~\cite{ctm}}  & \emph{ResNet18}${}^{\dag}$  & 64.12 \small{$\pm$ $0.82$} & 80.51 \small{$\pm$ $0.13$}  & 68.41 \small{$\pm$ $0.39$}  & 84.28 \small{$\pm$ $1.73$} \\\Xhline{1pt}

\textbf{DeepEMD-FCN}  & \emph{ResNet12}  & \textbf{66.50} \small{$\pm$ \textbf{0.80}} & \textbf{82.41} \small{$\pm$ \textbf{0.56}}  & \textbf{72.65} \small{$\pm$ \textbf{0.31}}  & \textbf{86.03} \small{$\pm$ \textbf{0.58}} \\ 

\textbf{DeepEMD-Grid}  & \emph{ResNet12}  & \textbf{67.83} \small{$\pm$ \textbf{0.29}} & \textbf{83.14} \small{$\pm$ \textbf{0.57}}  & \textbf{73.13} \small{$\pm$ \textbf{0.32}}  & \textbf{87.08} \small{$\pm$ \textbf{0.60}} \\ 

\textbf{DeepEMD-Sampling}  & \emph{ResNet12}  & \textbf{68.77} \small{$\pm$ \textbf{0.29}} & \textbf{84.13} \small{$\pm$ \textbf{0.53}}  & \textbf{74.29} \small{$\pm$ \textbf{0.32}}  & \textbf{86.98} \small{$\pm$ \textbf{0.60}} \\ 
\Xhline{1pt}



					
				\end{tabular*}
				
		\caption{ Results on \textbf{\emph{mini}ImageNet} and \textbf{\emph{tiered}ImageNet} datasets}
		\end{subtable}
		
		\end{minipage}

		\begin{minipage}{1\textwidth}
		\begin{minipage}[t]{0.5\textwidth}
\centering
			\begin{subtable}{1\textwidth}
				\resizebox{\textwidth}{!}{
					
					\begin{tabular}{lccc}
						\toprule[1pt]
						\multicolumn{1}{c}{\textbf{Method}} &\textbf{ Backbone} & \textbf{1-shot}        & \textbf{5-shot }       \\ \Xhline{1pt}
\textbf{\emph{cosine} classifier~\cite{closer}} & \emph{ResNet12} & 38.47 \small{$\pm$ $0.70$} & 57.67 \small{$\pm$ $0.77$} \\

\textbf{TADAM~\cite{TADAM}} & \emph{ResNet12} & 40.10 \small{$\pm$ $0.40$} & 56.10 \small{$\pm$ $0.40$} \\

\textbf{MetaOptNet~\cite{metaoptnet}} & \emph{ResNet12} &  41.10\small{$\pm$ $0.60$} & 55.5 \small{$\pm$ $0.60$} \\

\textbf{ProtoNet~\cite{proto}} & \emph{ResNet12} & 41.54 \small{$\pm$ $0.76$} & 57.08 \small{$\pm$ $0.76$} \\


\textbf{DC~\cite{dense}} & \emph{ResNet12} & 42.04 \small{$\pm$ $0.17$} & 57.05 \small{$\pm$ $0.16$} \\

\textbf{MatchNet~\cite{matchnet}} & \emph{ResNet12} & 43.88 \small{$\pm$ $0.75$} & 57.05 \small{$\pm$ $0.71$} \\

\textbf{MTL~\cite{yaoyao}} & \emph{ResNet12} &  45.10\small{$\pm$ $1.8$} & 57.6 \small{$\pm$ $0.9$} \\\Xhline{1pt}

\textbf{DeepEMD-FCN} & \emph{ResNet12} &  \textbf{46.60} \small{$\pm$ \textbf{0.26}} &  \textbf{63.22} \small{$\pm$ \textbf{0.71}} \\

\textbf{DeepEMD-Grid} & \emph{ResNet12} &  \textbf{45.23} \small{$\pm$ \textbf{0.26}} &  \textbf{61.39} \small{$\pm$ \textbf{0.76}} \\

\textbf{DeepEMD-Sampling} & \emph{ResNet12} &  \textbf{45.37} \small{$\pm$ \textbf{0.25}} &  \textbf{61.51} \small{$\pm$ \textbf{0.70}} \\\bottomrule[1pt]

						

					\end{tabular}
				}
				\caption{Results on \textbf{Fewshot-CIFAR100} dataset.}
			\end{subtable}
			\end{minipage}
			\begin{minipage}[t]{0.5\textwidth}
			\begin{subtable}{1\textwidth}
				\resizebox{\textwidth}{!}{
					\begin{tabular}{lccc}
						\toprule[1pt]
						
				\multicolumn{1}{c}{\textbf{Method}} &\textbf{ Backbone} & \textbf{1-shot}        & \textbf{5-shot }       \\ \Xhline{1pt}		
\textbf{ProtoNet~\cite{proto}} & \emph{ResNet12} & 66.09 \small{$\pm$ $0.92$} & 82.50 \small{$\pm$ $0.58$} \\	

\textbf{RelationNet~\cite{relation,closer}} & \emph{ResNet34}${}^{\dag}$ & 66.20 \small{$\pm$ $0.99$} & 82.30 \small{$\pm$ $0.58$} \\						

\textbf{DEML~\cite{Zhou2018deep}} & \emph{ResNet50}${}^{\dag}$ & 66.95 \small{$\pm$ $1.06$} & 77.11 \small{$\pm$ $0.78$} \\

\textbf{MAML~\cite{maml,closer}} & \emph{ResNet34}${}^{\dag}$ & 67.28 \small{$\pm$ $1.08$} & 83.47 \small{$\pm$ $0.59$} \\

\textbf{\emph{cosine} classifier~\cite{closer}} & \emph{ResNet12} &  67.30 \small{$\pm$ $0.86$} & 84.75 \small{$\pm$ $0.60$} \\




\textbf{MatchNet~\cite{matchnet}} & \emph{ResNet12} & 71.87 \small{$\pm$ $0.85$} & 85.08 \small{$\pm$ $0.57$} \\\Xhline{1pt}

\textbf{DeepEMD-FCN} & \emph{ResNet12} &  \textbf{77.14} \small{$\pm$ \textbf{0.29}} &  \textbf{88.98} \small{$\pm$ \textbf{0.49}} \\

\textbf{DeepEMD-Grid} & \emph{ResNet12} &  \textbf{77.64} \small{$\pm$ \textbf{0.29}} &  \textbf{89.25} \small{$\pm$ \textbf{0.53}} \\

\textbf{DeepEMD-Sampling} & \emph{ResNet12} &  \textbf{79.27} \small{$\pm$ \textbf{0.29}} &  \textbf{89.80} \small{$\pm$ \textbf{0.51}} \\
					\Xhline{1pt}	
					\end{tabular}
				}
			\caption{Results on  \textbf{Caltech-UCSD Birds-200-2011} dataset.}
			\end{subtable}

		\end{minipage}
	

	\label{table:soa}	
 	\end{minipage}

	
\end{table*}
